When Less is More: Investigating Data Pruning for Pretraining LLMs at Scale

Large volumes of text data have contributed significantly to the development of large language models (LLMs) in recent years. This data is typically acquired by scraping the internet, leading to pretraining datasets comprised of noisy web text. To date, efforts to prune these datasets down to a higher quality subset have relied on hand-crafted heuristics encoded as rule-based filters. In this work, we take a wider view and explore scalable estimates of data quality that can be used to systematically measure the quality of pretraining data. We perform a rigorous comparison at scale of the simple data quality estimator of perplexity, as well as more sophisticated and computationally intensive estimates of the Error L2-Norm and memorization. These metrics are used to rank and prune pretraining corpora, and we subsequently compare LLMs trained on these pruned datasets. Surprisingly, we find that the simple technique of perplexity outperforms our more computationally expensive scoring methods. We improve over our no-pruning baseline while training on as little as 30% of the original training dataset. Our work sets the foundation for unexplored strategies in automatically curating high quality corpora and suggests the majority of pretraining data can be removed while retaining performance.

==> tables/data.tex <==
\begin{table*}[htb]
\tiny
\centering
\caption{Data Points and their Calculated Perplexity}
\label{tab:data}
\resizebox{\textwidth}{!}{
\begin{tabular}{ |p{1cm}||p{1.5cm}|p{1.5cm}|p{5cm}|  }
 \hline
 \multicolumn{4}{|c|}{Perplexity Examples} \\
 \hline
 Model & Subset & Perplexity &Text\\
 \hline
 52B & Bottom 10\% & 1.171 & IF THE ARBITRATION AWARD IS EQUAL TO OR GREATER THAN THE\\
 \hline
 52B & Bottom 10\% & 2.179   & us when you contact us, sign-up for a customer account,\\
 \hline
 52B & Bottom 10\% & 14.047 & esthesiologist during a hernia repair to administer a blood thinning drug\\
 \hline
 52B & Middle 10\% & 103.958 & carry your burdens in love by giving you space to be honest \\
 \hline
 52B & Middle 10\% & 110.650 & on Vancouver Island in 2017 proved to be enough to hand a minority government \\
 \hline
 52B & Middle 10\% & 123.805 & I'm wrong but for now, let's examine something McCaffrey does so well for a running \\
 \hline
 52B & Top 10\%  & 284.992 & deep theological truths about the basic doctrines of the Bible, but\\
 \hline
 52B & Top 10\%  & 302.787 & 's Fashion Chic winning Best Female, CC, Club Winner 2018 and Greyhound SPECIALTY BEST IN SHOW!!!\\
 \hline
 52B & Top 10\%  & 342.559 & kind, and almost always just. That is, she was just when she understood things \\
 \hline
 Wikipedia & Bottom 10\%  & 1.170 & IF THE ARBITRATION AWARD IS EQUAL TO OR GREATER THAN THE \\
 \hline
 % Wikipedia & Bottom 10\%  & 1.170 & IF THE ARBITRATION AWARD IS EQUAL TO OR GREATER THAN THE \\
 % \hline
 % Wikipedia & Bottom 10\%  & 1.170 & IF THE ARBITRATION AWARD IS EQUAL TO OR GREATER THAN THE \\
\end{tabular}
}
\end{table*}
